A distributional simplicity bias in the learning dynamics of transformers

The remarkable capability of over-parameterised neural networks to generalise effectively has been explained by invoking a ``simplicity bias'': neural networks prevent overfitting by initially learning simple classifiers before progressing to more complex, non-linear functions. While simplicity biases have been described theoretically and experimentally in feed-forward networks for supervised learning, the extent to which they also explain the remarkable success of transformers trained with self-supervised techniques remains unclear. In our study, we demonstrate that transformers, trained on natural language data, also display a simplicity bias. Specifically, they sequentially learn many-body interactions among input tokens, reaching a saturation point in the prediction error for low-degree interactions while continuing to learn high-degree interactions. To conduct this analysis, we develop a procedure to generate \textit{clones} of a given natural language data set, which rigorously capture the interactions between tokens up to a specified order. This approach opens up the possibilities of studying how interactions of different orders in the data affect learning, in natural language processing and beyond.

==> settings.tex <==
\newcommand{\softmax}[1]{\text{softmax}\left(#1\right)}
\newcommand{\V}{|\mathbb{V}|}


% The following are the matplotlib default colours
% (useful for making references to colours in plots)
\definecolor{C0}{HTML}{1f77b4}
\definecolor{C1}{HTML}{ff7f0e}
\definecolor{C2}{HTML}{2ca02c}
\definecolor{C3}{HTML}{d62728}
\definecolor{C4}{HTML}{9467bd}
\definecolor{C5}{HTML}{8c564b}
\definecolor{C6}{HTML}{e377c2}
\definecolor{C7}{HTML}{7f7f7f}
\definecolor{C8}{HTML}{bcbd22}
\definecolor{C9}{HTML}{17becf}
\definecolor{gaussian}{HTML}{47908C}

\newtheorem{example}{Example}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{axiom}[theorem]{Axiom}
\newtheorem{cor}[theorem]{Corollary}
\newtheorem{prop}[theorem]{Proposition}
\newtheorem{claim}{Claim}
\newtheorem{assumption}{Assumption}

% Shorthands
\def\out{\text{out}}
\def\new{\text{new}}
\def\iid{\text{i.i.d.}}
\newcommand{\argmin}{\textrm{argmin}}

% Integral measures
\def\relu{\text{relu}}

% Special functions
\def\sign{\text{sign}}

\DeclareMathOperator{\cov}{\mathsf{cov}}
\DeclareMathOperator{\mmse}{\sf mmse}
\DeclareMathOperator{\pmse}{\sf pmse}
\DeclareMathOperator{\snr}{\sf snr}
\DeclareMathOperator{\npi}{\sf npi}
\DeclareMathOperator{\diag}{\mathrm{diag}}
\newcommand{\ka}{\kappa}
\newcommand{\sqD}{\sqrt{D}}
\newcommand{\sqP}{\sqrt{P}}
\newcommand{\EE}{\mathbb{E}\,}
\newcommand{\EEp}{\underset{+}{\mathbb{E}}\,}
\newcommand{\EEm}{\underset{-}{\mathbb{E}}\,}
\newcommand{\reals}{\mathbb{R}}
\newcommand{\integers}{\mathbb{N}}

\def\va{{\mathbf{a}}}
\def\vh{{\mathbf{h}}}
\def\vm{{\mathbf{m}}}
\def\vv{{\mathbf{v}}}
\def\vw{{\mathbf{w}}}
\def\vx{{\mathbf{x}}}
\def\vz{{\mathbf{z}}}

